Complex Reading Comprehension Through Question Decomposition

Multi-hop reading comprehension requires not only the ability to reason over raw text but also the ability to combine multiple evidence. We propose a novel learning approach that helps language models better understand difficult multi-hop questions and perform "complex, compositional" reasoning. Our model first learns to decompose each multi-hop question into several sub-questions by a trainable question decomposer. Instead of answering these sub-questions, we directly concatenate them with the original question and context, and leverage a reading comprehension model to predict the answer in a sequence-to-sequence manner. By using the same language model for these two components, our best seperate/unified t5-base variants outperform the baseline by 7.2/6.1 absolute F1 points on a hard subset of DROP dataset.

==> sec6-limit.tex <==
%!TEX ROOT = ./acl2021.tex
% \section*{Limitations}
% Though our proposed methods can be applied on other machine reading comprehension datasets, the experiments in this paper only focus on a hard partition from the DROP dataset. 
% Moreover, our technique only employs one specific LM, T5-base, to conduct experiments. 
% Experimenting with other T5 models and LMs such as GPT-3 remains our future work. 
% On the one hand, employing LMs with different sizes, such as T5-small or T5-large, can have an in-depth view about LMs with different parameters.
% On the other hand, limitations also exist in experiment lacking of using different kinds of LMs pretrained using different loss functions, such as GPT-3 and BART. 

==> sec7-appen.tex <==
%!TEX ROOT = ./acl2021.tex
% \clearpage
% \newpage
% \appendix
% \section{Appendix}
% \label{sec6-appen}
